Vision6D: 3D-to-2D Interactive Visualization and Annotation Tool for 6D Pose Estimation

Accurate 6D pose estimation has gained more attention over the years for robotics-assisted tasks that require precise interaction with physical objects. This paper presents an interactive 3D-to-2D visualization and annotation tool to support the 6D pose estimation research community. To the best of our knowledge, the proposed work is the first tool that allows users to visualize and manipulate 3D objects interactively on a 2D real-world scene, along with a comprehensive user study. This system supports robust 6D camera pose annotation by providing both visual cues and spatial relationships to determine object position and orientation in various environments. The annotation feature in Vision6D is particularly helpful in scenarios where the transformation matrix between the camera and world objects is unknown, as it enables accurate annotation of these objects' poses using only the camera intrinsic matrix. This capability serves as a foundational step in developing and training advanced pose estimation models across various domains. We evaluate Vision6D's effectiveness by utilizing widely-used open-source pose estimation datasets Linemod and HANDAL through comparisons between the default ground-truth camera poses with manual annotations. A user study was performed to show that Vision6D generates accurate pose annotations via visual cues in an intuitive 3D user interface. This approach aims to bridge the gap between 2D scene projections and 3D scenes, offering an effective way for researchers and developers to solve 6D pose annotation related problems. The software is open-source and publicly available at https://github.com/InteractiveGL/vision6D.

==> trashcan.tex <==
% \begin{figure*}[!ht]
%      %--- First block of two images
%     \begin{minipage}[t]{0.45\textwidth}
%         \begin{minipage}{0.95\textwidth}
%             \includegraphics[width=\textwidth]{exmaple.png}
%         \end{minipage}\hspace{-0.5em}
%         \centering
%         NASA-TLX Evaluation
%     \end{minipage}
%     \hfill
%     %--- Second block of two images
%     \begin{minipage}[t]{0.45\textwidth}
%         \begin{minipage}{0.95\textwidth}
%             \includegraphics[width=\textwidth]{exmaple.png}
%         \end{minipage}\hspace{-0.5em}
%         \centering
%         SUS Evaluation
%     \end{minipage}
%     \hfill
%     \caption{\textbf{User Feedback.} We present user feedback using two standardized evaluation metrics: NASA-TLX for assessing cognitive workload and task difficulty, and SUS for measuring system usability.}
%     \label{fig:user_feedback}
% \end{figure*}



% \subsubsection{Learning Curve Analysis}
% We assess the change in annotation time across repeated trials for the same sample, indicating whether user annotate faster with practice. The learning curve analysis, shown in Figure~\ref{fig:learning_curve_analysis}, revealing that annotation time generally decrease with successive annotations, indicating that users tend to become more efficient as they gain experience.

% \begin{figure*}[ht]
%      %--- First block of two images
%     \begin{minipage}[t]{0.45\textwidth}
%         \begin{minipage}[c]{0.05\textwidth}
%             \centering
%             \rotatebox{90}{Time Spent (seconds)}
%         \end{minipage}
%         \begin{minipage}{0.95\textwidth}
%             \includegraphics[width=\textwidth]{exmaple.png}
%         \end{minipage}\hspace{-0.3em}
%     \end{minipage}
%     \hfill
%     %--- Second block of two images
%     \begin{minipage}[t]{0.45\textwidth}
%         \begin{minipage}[c]{0.05\textwidth}
%             \centering
%             \rotatebox{90}{Time Spent (seconds)}
%         \end{minipage}
%         \begin{minipage}{0.95\textwidth}
%             \includegraphics[width=\textwidth]{exmaple.png}
%         \end{minipage}\hspace{-0.3em}
%     \end{minipage}
%     \hfill

%     %--- First block of two images
%     \begin{minipage}[t]{0.45\textwidth}
%         \begin{minipage}[c]{0.05\textwidth}
%             \centering
%             \rotatebox{90}{ADD Metric (in mm)}
%         \end{minipage}
%         \begin{minipage}{0.95\textwidth}
%             \includegraphics[width=\textwidth]{exmaple.png}
%         \end{minipage}\hspace{-0.3em}

%         \centering
%         Linemod Dataset
%     \end{minipage}
%     \hfill
%     %--- Second block of two images
%     \begin{minipage}[t]{0.45\textwidth}
%         \begin{minipage}[c]{0.05\textwidth}
%             \centering
%             \rotatebox{90}{ADD Metric (in mm)}
%         \end{minipage}
%         \begin{minipage}{0.95\textwidth}
%             \includegraphics[width=\textwidth]{exmaple.png}
%         \end{minipage}\hspace{-0.3em}
    
%         \centering
%         HANDAL Dataset
%     \end{minipage}
%     \hfill
    
%     \caption{\textbf{Learning Curve Analysis.} We assess user learning progress by analyzing the annotation time across three trials per sample, measuring improvements in efficiency and adaptation to Vision6D.}
%     \label{fig:learning_curve_analysis}
% \end{figure*}

% talk about the differences between Blender and Unity
Applications like Blender and Unity emphasize user interaction, making complex tasks such as object manipulation, animation, and rendering more approachable and fun. Blender’s GUI simplifies the creation of high-quality visual effects by offering intuitive tools for manipulating 3D models and camera view angles, allowing developers to focus more on problem-solving and less on technical complexity. Similarly, Unity's visual and component-based system allows users to design complex interactions and animations without extensive programming knowledge, making the development process more accessible and efficient.

This tool unleashes the possibility to integrate 2D image data with the corresponding 3D models, showing real-time manipulation of the 6D camera poses.

which represent how the scene would appear in an image captured by the specific camera


%This design allows for an extensive analysis of how consistently a single participant can replicate their annotations (intra-personal consistency) as well as how annotations vary across different participants (inter-personal variability). Consequently, the dataset organization provides a comprehensive evaluation of both the pose annotating precision and reliability of the Vision6D tool in generating accurate 6D pose annotations in real-world scenarios.


% How 6D pose annotations have been created in the past. Many of them perform manual trial and error by modifying a pose numerically and updating a render to verify.
% Can be challenging and exporting camera poses are not provided or supported by many annotation tools

% Aruco markers are commonly used to annotate frames -- however, this type of solution might not be applicable to all domains (e.g. medical). Additionally, it can be very time consuming to create poses for a video without using an interactive tool
% Need of a efficient and robust tool for annotation 6D poses
% Despite the recent advancements in 6D pose estimation using deep-learning-based methods, significant gaps remain between traditional 6D pose annotation methods, existing 3D GUIs, and the need for efficient camera pose annotation. Traditional pose annotation techniques rely heavily on synthesizing camera pose datasets or utilizing fiducial markers, which present various challenges in authentic scenarios. ArUco markers for pose annotation effectively determine camera poses in structured and controlled environments. These markers provide a reliable way to generate 6D pose annotations when the markers are visible. However, this approach has several limitations. First, fiducial markers like ArUco boards may not be applicable in all domains. For example, in medical applications, placing markers in surgical scenes or other clinical environments is often impractical or infeasible. Additionally, the time and effort required to set up markers and ensure their visibility throughout a recording session can make this method inflexible, particularly for long or complex scenes. Manually rendering 6D camera poses for the annotations frame by frame without the assistance of an interactive tool is time-consuming. In situations where real-time adjustments are needed, such as in surgical scenes or autonomous navigation, the process of manually modifying poses numerically and then updating the corresponding renders to verify the poses can be inefficient. Though commonly used in the research community, the trial-and-error approach is unsuitable for large dataset creation or scenarios requiring rapid feedback. The lack of interactivity slows the annotation process, resulting in an inefficient workflow.

% Useful resources for camera projection
% https://github.com/polygon-software/python-visual-odometry/blob/master/Chapter%203%20-%20Camera%20Projection.ipynb

% Talk about image formation, camera intrinsics and extrinsics. Math model (diagram and a screenshot)
% Talk about projection and rendering.

% Overview of the system including the main 3 components in the application: 3D scene display, Main Panel, and the Output panel. All of these combined provide a solution for 6D pose annotation and export.

% Menu Panel (IO inteface for saving and writing images, meshes, and poses)
% Control panel (Apply changes to 3D scene such as camera intrinsics, etc)
% Display panel (track and manage of 3D objects within the 3D scene display)

 % This intuitive Display Subpanel allows for real-time interaction with objects, supporting future efficient pose adjustments and alignment in 3D Scene Display.

 
% References
% [1] https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=10418508
% [2] https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=10453452
% [3] https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=10418108
% [4] https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9847102
% [5] https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9920664

% This evaluation provides an in-depth understanding of how Vision6D provides reliable pose annotations and how it handles subjective annotation differences, ultimately contributing to future research and practical applications.

%By comparing participant annotations with ground-truth poses, we measure how closely manual annotations align with dataset benchmarks, highlighting the tool’s reliability and usability across different users. 

% It also reveal potential avenues for further improvements, ultimately providing a well-rounded evaluation of the overall user experience.

% User click on the 3D object and there will automatically 2D projection pixel locations
% Talk about 2D-3D correspondence.
% Future possible feature of assisted pose estimation in video by using initial pose frame and camera localization methods to estimate interframe camera movement and compute next frames' target object pose. Then the user can simply refine instead of completely annotate target object pose from scratch.

% Contributions
%% Vision6D, mainly focus on the first frame regitration, in some senarios, the pre-recorded videos does not have enough camera movements to apply the state-of-the-art pose estimation skills. e.g. in cochlear implant surgery.
%% Lightweight Desktop application for annotating 

==> trashcan/trashcan.tex <==
Additionally, we aim to develop a web-based or cross-platform version of Vision6D to minimize system dependencies and improve accessibility across different operating systems. 

% Vision6D has been primarily developed for the Windows operating system, we tested its performance and compatibility on Linux and MacOS to assess its cross-platform functionality. Our results indicate that the system runs smoothly on Linux, maintaining full functionality without performance issues. However, on MacOS, certain features are restricted due to OS-specific constraints, including differences in system-level dependencies and hardware compatibility. For future work, we plan to address MacOS-specific constraints by optimizing platform-independent rendering and enhancing compatibility with MacOS.
